Transforming LLMs into Cross-modal and Cross-lingual Retrieval Systems

Large language models (LLMs) are trained on text-only data that go far beyond the languages with paired speech and text data. At the same time, Dual Encoder (DE) based retrieval systems project queries and documents into the same embedding space and have demonstrated their success in retrieval and bi-text mining. To match speech and text in many languages, we propose using LLMs to initialize multi-modal DE retrieval systems. Unlike traditional methods, our system doesn't require speech data during LLM pre-training and can exploit LLM's multilingual text understanding capabilities to match speech and text in languages unseen during retrieval training. Our multi-modal LLM-based retrieval system is capable of matching speech and text in 102 languages despite only training on 21 languages. Our system outperforms previous systems trained explicitly on all 102 languages. We achieve a 10% absolute improvement in Recall@1 averaged across these languages. Additionally, our model demonstrates cross-lingual speech and text matching, which is further enhanced by readily available machine translation data.

==> latex/data/seen_vs_unseen_asr_retrieval_wer.tex <==

\definecolor{RYB0}{RGB}{237,248,251}
\definecolor{RYB1}{RGB}{178,226,226}
\definecolor{RYB2}{RGB}{102,194,164}
\definecolor{RYB3}{RGB}{35,139,69}

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[scale=0.7]
    \begin{axis}[
      xbar, % Use xbar for horizontal bars
      bar width=0.5cm,
      enlarge y limits={abs=0.2cm}, % Adjust the spacing between bars
      symbolic y coords={Seen (20 Lang.), Unseen (82 Lang.), All (102 Lang.), mSLAM DE(102 Lang.)},
      ytick=\empty, % Remove y ticks
      xlabel={WER},
      title={ASR Retrieval},
      legend style={at={(0.97,0.2)}, anchor=east, legend columns=1, font=\small, fill opacity=0.8, reverse legend}, % Set fill opacity
      grid=major,
    ]
      \addplot[fill=RYB3] coordinates {(5.29,Seen (20 Lang.))};
      \addplot[fill=RYB2] coordinates {(15.94,Unseen (82 Lang.))};
      \addplot[fill=RYB1] coordinates {(13.85,All (102 Lang.))};
      \addplot[fill=RYB0, postaction={pattern=north east lines}] coordinates {(14.6,mSLAM DE (102 Lang.))};
      \legend{Seen (20 Lang.), Unseen (82 Lang.), All (102 Lang.), mSLAM DE (102 Lang.)}
    \end{axis}
  \end{tikzpicture}
  \caption{mSLAM DE Results for Different Language Sets (Horizontal Bar Plot)}
  \label{fig:seen_vs_unseen_wer}
\end{figure}

==> latex/fleurs_s2tt_bleu_combined_comparisons.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
               & \emph{\# Langs.} & \emph{CV}    & \emph{CV + WM} \\ \midrule
Afro-Asiatic   & 7         & 20.76 & 20.82   \\
Atlantic-Congo & 15        & 18.47 & 19.16   \\
Austro-Asiatic & 3         & 16.43 & 19.88   \\
Austronesian   & 6         & 20.95 & 22.25   \\
Dravidian      & 4         & 17.17 & 20.09   \\
Indo-European  & 51        & 28.46 & 31.11   \\
Japonic        & 1         & 23.1  & 25.08   \\
Kartvelian     & 1         & 18.77 & 21.79   \\
Koreanic       & 1         & 19.19 & 22.42   \\
Kra-Dai        & 1         & 18.7  & 22.31   \\
Mongolic       & 1         & 19.86 & 22.28   \\
Nilo-Saharan   & 1         & 15.13 & 18.03   \\
Sino-Tibetan   & 3         & 18.96 & 24.2    \\
Turkic         & 4         & 20.18 & 21.76   \\
Uralic         & 3         & 21.74 & 23.32   \\ \bottomrule
\end{tabular}%
}
\caption{BLEU scores for zero-shot FLEURS S2TT retrieval broken down by language family. Extended PaLM 2 was trained on Common Voice (\textbf{CV}) or a mix of Common Voice and Wikimatrix (\textbf{CV + WM}). }
\label{tab:my-table}
\end{table}

==> latex/recall_by_tokenizer.tex <==
\begin{table}[t]
  \centering
\resizebox {\linewidth} {!} {
  \begin{tabular}{lrrr}
    \toprule
    &\multicolumn{3}{c}{\textit{R@1} $\uparrow$} \\
    \cmidrule{2-4}
    {Language Group (\#)} &  mSLAM DE & \multicolumn{2}{c}{PaLM 2 DE} \\
    \cmidrule{3-4}
    & {\cite{conneau2023fleurs}} & {USM-v1} &  {USM-v2}\\
    \midrule
    Afro-Asiatic (7) & 73.67 & \textbf{90.82}  & 87.75 \\
    Atlantic-Congo (14) & \textbf{86.77} & 79.47 & 76.85\\
    Austro-Asiatic (2) & 47.90 & 41.71 & \textbf{91.50} \\
    Austronesian (6) & 75.50 & 85.74  & \textbf{96.13} \\
    Dravidian (4) & 65.70 & \textbf{90.46} & 84.87 \\
    Indo-European (51) & 84.62 & \textbf{92.38} & 90.87 \\
    Japonic (1) & 5.80 & 63.23  & \textbf{96.95} \\
    Kartvelian (1) & 70.50 & 74.57 & \textbf{100.00} \\
    Koreanic (1) & 5.20 & 45.81 & \textbf{52.36} \\
    Kra-Dai (2) & 3.20 & 37.12 & \textbf{90.66} \\
    Mongolic (1) & 70.70 & 98.10 & \textbf{98.66} \\
    Nilo-Saharan (1) & 91.00 & \textbf{94.53} & 23.31 \\
    Sino-Tibetan (3) & 3.40 & 61.91 & \textbf{90.66} \\
    Turkic (5) & 81.28 & \textbf{91.89} & 65.27 \\
    Uralic (3) & 91.40 & \textbf{93.38} & 90.41\\
    \midrule
    All (102) & 76.9 & 86.15 & \textbf{86.60} \\
    
    \bottomrule
  \end{tabular}
  }
  \caption{FLEURS S2T (\emph{R@1}) performance broken down by language groups. Bold represents better performance. We report \emph{R@1} for USM-v1 and USM-v2 audio tokenizers for PaLM 2 DE. These are the same audio tokenizers used in \citet{rubenstein2023audiopalm}.} 
  \label{tab:recall_per_tokenizer}
\end{table}



